SAILOR: A Scalable and Energy-Efficient Ultra-Lightweight RISC-V for IoT Security

Recently, RISC-V has contributed to the development of IoT devices, requiring architectures that balance energy efficiency, compact area, and integrated security. However, most recent RISC-V cores for IoT prioritize either area footprint or energy efficiency, while adding cryptographic support further compromises compactness. As a result, truly integrated architectures that simultaneously optimize efficiency and security remain largely unexplored, leaving constrained IoT environments vulnerable to performance and security trade-offs. In this paper, we introduce SAILOR, an energy-efficient and scalable ultra-lightweight RISC-V core family for cryptographic applications in IoT. Our design is modular and spans 1-, 2-, 4-, 8-, 16-, and 32-bit serialized execution data-paths, prioritizing minimal area. This modular design and adaptable data-path minimizes the overhead of integrating RISC-V cryptography extensions, achieving low hardware cost while significantly improving energy efficiency. We validate our design approach through a comprehensive analysis of area, energy, and efficiency trade-offs. The results surpass state-of-the-art solutions in both performance and energy efficiency by up to 13x and reduce area by up to 59 %, demonstrating that lightweight cryptographic features can be added without prohibitive overhead, and that energy- or area-efficient designs need not compromise performance.

==> keywords.tex <==
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
IEEE, IEEEtran, journal, \LaTeX, paper, template.
\end{IEEEkeywords}

==> sections/08_acknowledgment.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}


==> sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
\begin{IEEEbiography}[{\includegraphics[trim={1cm 0 8cm 0}, width=1in,height=1.25in,clip,keepaspectratio]{photos/ewert_selfie.jpg}}]{Christian Ewert} 
	received his B.Sc. and M.Sc. in Computer Engineering from the University of Rostock and Leibniz University Hanover (LUH), Germany, respectively. Since 2021, he has been a research assistant and Ph.D. student member of the Trustworthiness Research Group at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany. His research interests include secure processor design, secure and lightweight SoC design, and hardware design for security applications in resource-constrained IoT environments.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Tim.JPG}}]{Tim Hardow} received his B.Sc. in Computer Science from the \glqq Universit\"at zu L\"ubeck\grqq. He is currently pursuing the M.Sc. in Computer Science and working as a research engineer at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq. The focus of his work is on RISC-V processor design and cryptographic accelerators.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/pic_fritsch.pdf}}]{Melf Fritsch}
received the B.Sc. in Computer Science from the \glqq Universit\"at zu L\"ubeck\grqq, Germany, in 2023.
He is currently pursuing the M.Sc. in Computer Science and is working as a student assistant at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany, where he is also conducting his master's thesis research. His research interests include digital hardware design and RISC-V-based architectures.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[trim={5cm 11cm 7cm 5cm}, width=1in,height=1.25in,clip,keepaspectratio]{photos/pic_dietrich.jpg}}]{Leon Dietrich}
received his M.Sc.~in Robotics from \glqq Universit\"at zu L\"ubeck\grqq, Germany. Since 2022, he has been a research assistant at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany, and is a member of the Trustworthiness Research Group. His current research activities focus on hardware acceleration of cryptographic algorithms as well as required interfacing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/pic_slides_Strunck.jpg}}]{Henrik Strunck} received his M.Sc. in IT Security and his B.Sc. in Computer Science from \glqq Universit\"at zu L\"ubeck\grqq, Germany. Since 2023, he has been a research assistant and Ph.D. student at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany, and is a member of the Trustworthiness Research Group. His current research interests lie in hardware security, focusing on hardware roots of trust and embedded system security in RISC-V ecosystems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/rainer-2.png}}]{Rainer Buchty}
	received the Diploma and Ph.D. degrees in computer science from TU Munich, Germany, in 1997 and 2002, respectively. In 2019, he joined the \glqq Universit\"at zu L\"ubeck\grqq, Germany, as the Project and Research Manager, with a focus on processor and systems design with Prof. Berekovic. His past experiences include academic positions at KIT, the University of Jena, and TU Braunschweig, including its associated technology transfer company iTUBS GmbH, a temporary professorship at the University of Tübingen, as well as industrial experiences at AMD GmbH, Munich, and Bell Labs, Holmdel, NJ, USA, and their respective spin-offs Vantis GmbH and Agere Systems.\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/mladen.png}}]{Mladen Berekovic}
	(Member, IEEE) received the Ph.D. degree in circuit design for signal processing systems from the Leibniz University of Hannover, Germany. After the Ph.D. studies, he worked on processor design at IBM and led research teams in reconfigurable computing and mobile system design at the Interuniversity Microelectronics Centre (IMEC), Belgium. He is currently the Director of the Institute for Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany. Before that, he was the Chair of the Computer Engineering Group and the Intel Chair of VLSI design, both at the Technical University of Braunschweig (TUBS), Germany. His research interests include circuit and system design for safe, reliable, and secure autonomous systems.\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/saleh.png}}]{Saleh Mulhem}
	received the Ph.D. degree in cryptographic engineering from the Technical University of Braunschweig (TUBS), Germany. In 2015, he was a Ph.D. student member of the Reliability and Security Research Group at the Institute of Computer and Network Engineering, TUBS. During his Ph.D. studies, he received a full research grant from the German Academic Exchange Service (DAAD). Since 2020, he has led the Trustworthiness Research Group at the Institute of Computer Engineering, \glqq Universit\"at zu L\"ubeck\grqq, Germany. His research interests include trustworthy computing, secure SoC design, trustworthy hardware accelerators, and embedded system security.\end{IEEEbiography}




% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
